From One to All: Learning to Match Heterogeneous and Partially Overlapped Graphs

Recent years have witnessed a flurry of research activity in graph matching, which aims at finding the correspondence of nodes across two graphs and lies at the heart of many artificial intelligence applications. However, matching heterogeneous graphs with partial overlap remains a challenging problem in real-world applications. This paper proposes the first practical learning-to-match method to meet this challenge. The proposed unsupervised method adopts a novel partial OT paradigm to learn a transport plan and node embeddings simultaneously. In a from-one-to-all manner, the entire learning procedure is decomposed into a series of easy-to-solve sub-procedures, each of which only handles the alignment of a single type of nodes. A mechanism for searching the transport mass is also proposed. Experimental results demonstrate that the proposed method outperforms state-of-the-art graph matching methods.

==> sections/bcd.tex <==
\begin{algorithm}[t]
	\caption{\name{}-refine}\label{alg:fota_refine}
	\begin{algorithmic}[1]
		\State {\textbf{Input:}} $L$ outer-loops, $M$ rounds, $K$, $\alpha$, $\beta$, graphs $\GM^\src$ and $\GM^\tar$.
		\State {\textbf{Output:}} Correspondence set $\DM$.
		\State Calculate $\CB^\src$ and $\CB^\tar$ as Eq. (\ref{eq:constant_proximity}).
		\State Obtain transport mass for each type $\bB$ via Algorithm \ref{alg:linesearch}.
		\State Initialize $\ZB^\src$ and $\ZB^\tar$ via SVD for $\CB^\src$ and $\CB^\tar$ respectively.
		\For{$l=1,2,\dots,L$}
		\State $r=l\mod|\TM|$
		\For{$m=1,\dots,M$}
		\State Update transport plan by solving (\ref{eq:bcd_trans}).
		\State Update node embeddings by solving (\ref{eq:embedding subproblem}).
		\EndFor
		\State $\hat\TB^{r}=\hat\TB^{r,(M)}$.
		\EndFor
		\State $\hat{\TB}=\sum_{r=1}^{|\TM|}\hat\TB^{r}$.
		\State $\tilde{\TB}=[\hat{\TB},\muB^\src-\hat{\TB}\oneB]$.
		\State Initialize correspondence set $\DM=\emptyset$.
		\For{$i\in\{1,\dots,|\VM^\src|\}$}
		\State $i'=\arg\max_{i'} \tilde{T}_{ii'}$.
		\If{$i'\neq(|\VM^\tar|+1)$}
		\State $\DM=\DM\cup\{(i,i')\}$.
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}

The matching can be further refined after all types are matched.
Specifically, the optimization problem (\ref{eq:objective}) can be decomposed into $|\TM|$  \subproblems{} given by Eq. (\ref{eq:general_decomp}), which can be solved by alternating optimization, that is, alternatingly updating the transport plan by solving
\begin{equation}\label{eq:bcd_trans}
	\begin{aligned}
		\min_{\TB^{r}\in\Pi^{b_r}\big(\muB^{\src,r},\muB^{\tar,r}\big)}&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}^{r}T_{jj'}^{r}\\
		+&2\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}^{r}\Big(\sum_{r_1\neq r}\hat{T}_{jj'}^{r_1}\Big)\\
		+&\alpha\sum_{ii'}-\kappa\big(\zB_{i}^{\src,(m)},\zB_{i'}^{\tar,(m)}\big)T_{ii'}^{r},
	\end{aligned}
\end{equation}
where $\ZB^{\src,(m)}$ and $\ZB^{\tar,(m)}$ are the current node embeddings, and updating the node embeddings by solving problem (\ref{eq:embedding subproblem}).
Note that problem (\ref{eq:pot}) is a special case of (\ref{eq:bcd_trans}).
We summarize this variant of \name{} in Alg. \ref{alg:fota_refine}.
%Each loop $l$ is analog to a single round of block coordinate descent.


==> sections/proof.tex <==
%\paragraph{Proof of Theorem \ref{thm:noisy colored isomorphic graphs}.}
%
%By the definition, we have
%\begin{equation}
%	\begin{aligned}
%		&S_{i\pi^*(i)}(\TB^{*,r},\YB^{*,(r-1)},0)\\
%		=&\sum_{j=1}^{|\VM^\src|}(B_{ij}^\src-B_{\pi^*(i)\pi^*(j)}^\tar)^2T^{*,r}_{j\pi^*(j)}+2\sum_{j=1}^{|\VM^\src|}
%	\end{aligned}
%\end{equation}
%
%\begin{flushright}
%	$\blacksquare$
%\end{flushright}
We restate Proposition \ref{prop:model_decomposition} here for convenience.

\primeproposition*

\paragraph{Proof of Proposition \ref{prop:model_decomposition}.}
Substituting $\TB=\sum_{r=1}^{|\TM|}\TB^{r}$ into the objective of (\ref{eq:objective}), we have
\begin{equation*}
	\begin{aligned}
		&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}T_{jj'}+\alpha\sum_{ii'}-\kappa(\zB_{i}^{\src},\zB_{i'}^{\tar})T_{ii'}\\
		&+\beta\big(R(\ZB^\src)+R(\ZB^\tar)\big)\\
		=&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2\Big(T_{ii'}^{r}+\sum_{r_1\neq r}T_{ii'}^{r_1}\Big)\Big(T_{jj'}^{r}+\sum_{r_1\neq r}T_{jj'}^{r_1}\Big)\\
		-&\alpha\sum_{ii'}\kappa(\zB_{i}^{\src},\zB_{i'}^{\tar})\Big(T_{ii'}^{r}+\sum_{r_1\neq r}T_{ii'}^{r_1}\Big)\\
		+&\beta\big(R(\ZB^\src)+R(\ZB^\tar)\big)\\
		=&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}^{r}T_{jj'}^{r}-\alpha\sum_{ii'}\kappa(\zB_{i}^{\src},\zB_{i'}^{\tar})T_{ii'}^{r}\\
		+&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}^{r}\Big(\sum_{r_1\neq r}T_{jj'}^{r_1}\Big)\\
		+&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2\Big(\sum_{r_1\neq r}T_{ii'}^{r_1}\Big)T_{jj'}^{r}\\
		+&\beta\big(R^r(\ZB^{\src,r})+R^r(\ZB^{\tar,r})\big)+C,
	\end{aligned}
\end{equation*}
where $C$ is the sum of the terms irrelevant to $\TB^{r}$, $\ZB^{\src,r}$ and $\ZB^{\tar,r}$.
Because $C_{ij}^\src=C_{ji}^\src$ and $C_{i'j'}^\tar=C_{j'i'}^\tar$ for all $i,j\in\VM^\src$ and $i',j'\in\VM^\tar$,
dropping the irrelevant term $C$ and switching the order of $i$ and $j$ and the order of $i'$ and $j'$,
the optimization problem of the $r$\textsuperscript{th} \subprocedure{} is
\begin{equation}\label{eq:general_decomp}
	\begin{aligned}
		\min_{\TB^{r},\ZB^{\src,r},\ZB^{\tar,r}}&\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}^{r}T_{jj'}^{r}\\
		+&2\sum_{ii'jj'}(C_{ij}^\src-C_{i'j'}^\tar)^2T_{ii'}^{r}\Big(\sum_{r_1\neq r}\hat{T}_{jj'}^{r_1}\Big)\\
		+&\alpha\sum_{ii'}-\kappa(\zB_{i}^{\src},\zB_{i'}^{\tar})T_{ii'}^{r}\\
		+&\beta\big(R^r(\ZB^{\src,r})+R^r(\ZB^{\tar,r})\big),
	\end{aligned}
\end{equation}
such that $\TB^{r}\in\Pi^{b_r}\big(\muB^{\src,r},\muB^{\tar,r}\big)$.
Since we first match one type of nodes and gradually match other types, $\hat{\TB}^{a}=\zeroB$ for $a>r$ and we have the result.
\begin{flushright}
	$\blacksquare$
\end{flushright}
